Progress in the determination of Mellin moments of the pion LCDA using the HOPE method

The pion light-cone distribution amplitude (LCDA) is a central non-perturbative object of interest for the calculation of high-energy exclusive processes in quantum chromodynamics. In this article, we discuss the calculation of the second and fourth Mellin moment of the pion LCDA using a heavy-quark operator product expansion. The resulting value for the second Mellin moment is $ \langle{ \xi^2 }\rangle(\mu = 2~\text{GeV})= 0.210 \pm 0.013\text{ (stat.)} \pm 0.034\text{ (sys.)}$. This result is compatible with those from previous determinations of this quantity.

==> app-order-a.tex <==
\section{Symmetry Constraints on Matrix Element}


\subsection{Lorentz Invariant Decomposition}\label{app:lor_invar_decomp}
The derivation of the $\mathcal{O}(a)$ improvement relies on the symmetry properties of the hadronic amplitude that is constructed. The momentum-space hadronic amplitude is defined as 
%
\begin{equation}
  V^{\mu\nu}(p,q)=\int d^4z \, e^{-iq\cdot z}\bra{\Omega}|\mathcal{T}\{J^\mu(z/2)J^\mu(-z/2)\}\ket{\pi(\mathbf{p})} \, .
  \label{hadronic-tensor}
\end{equation}
%
The time-momentum representation of this amplitude, $R^{\mu\nu}(\tau, \mathbf{p}, \mathbf{q})$, is
obtained by performing a Fourier transform in the Euclidean momentum $q_4$:
%
\begin{equation}
\begin{split}
  R^{\mu\nu}(\tau,\mathbf{p},\mathbf{q})&=\int \frac{dq_4}{(2\pi)} e^{-iq_4\tau}V^{\mu\nu}(p,q) \, .
\end{split}
\end{equation}
%
In momentum-space, the most general Lorentz covariant form of the amplitude, $V^{\mu\nu}(p,q)$, is
%
\begin{equation}
  V^{\mu\nu}(p,q)=a_1 p^\mu p^\nu +a_2 p^\mu q^\nu + a_3 q^\mu p^\nu +a_4 q^\mu q^\nu+ a_5 g^{\mu\nu} + a_6 \epsilon^{\mu\nu\alpha\beta}p_\alpha q_\beta \, ,
  \label{tensor-decomposition}
\end{equation}
%
where $a_{i}$ are scalar functions of the invariants $q^2$, $p^2$ and $p\cdot q$, that is,
%
\begin{equation}
  a_i=a_i(p^2,q^2,p\cdot q) \, .
\end{equation}
%
Applying a parity transformation $\mathcal{P}$ to the hadronic amplitude gives
%
\begin{equation}
\begin{split}
  V^{\mu\nu}(p,q)&=\int d^4z \, e^{-i{q}\cdot {z}}\bra{0}|\mathcal{P}^\dagger\mathcal{P}\mathcal{T}\{J^\mu(\mathbf{z}/2,z_4/2)\mathcal{P}^\dagger\mathcal{P}J^\nu(-\mathbf{z}/2,-z_4/2)\}{\mathcal{P}^\dagger\mathcal{P}}\ket{\pi(\mathbf{p})}
\\
&={-}(-1)^\mu(-1)^\nu\int d^4z e^{-i q \cdot z}\bra{0}|\mathcal{T}\{J^\mu(-\mathbf{z}/2,z_4/2)J^\nu(\mathbf{z}/2,-z_4/2)\}\ket{\pi(-\mathbf{p})}
\\
&={-}(-1)^\mu(-1)^\nu V^{\mu\nu}(\tilde{p},\tilde{q}) \, ,
\end{split}
\end{equation}
%
where for simplicity the notation $\tilde{k}=(-\mathbf{k},p^4)$ has been introduced and
%
\begin{equation}
(-1)^\mu\equiv
\begin{cases}
-1,~\text{for}~\mu=1,2,3
\\
\hphantom{-}1,~\text{for}~\mu=4
\end{cases} \, .
\end{equation}
%
Applying these transformations to the terms in the amplitude decomposition, Eq.~\ref{tensor-decomposition}, gives
%
\begin{equation}
\begin{split}
a_1 p^\mu p^\nu +a_2 p^\mu q^\nu &+ a_3 q^\mu p^\nu +a_4 q^\mu q^\nu+ a_5 g^{\mu\nu} + a_6 \epsilon^{\mu\nu\alpha\beta}p_\alpha q_\beta
\\
&=-(-1)^\mu(-1)^\nu a_1 \tilde{p}^\mu \tilde{p}^\nu -(-1)^\mu(-1)^\nu a_2 \tilde{p}^\mu \tilde{q}^\nu -(-1)^\mu(-1)^\nu  a_3 \tilde{q}^\mu \tilde{p}^\nu -(-1)^\mu(-1)^\nu a_4 \tilde{q}^\mu \tilde{q}^\nu
\\
&-(-1)^\mu(-1)^\nu a_5 g^{\mu\nu} -(-1)^\mu(-1)^\nu a_6 \epsilon^{\mu\nu\alpha\beta}\tilde{p}_\alpha \tilde{q}_\beta \, .
\end{split}
\end{equation}
%
Noting that $p^\mu =(-1)^\mu \tilde{p}^\mu$, one may conclude all terms but $a_6$ vanish, and thus the most general form of the amplitude is
%
\begin{equation}
  V^{\mu\nu}(p,q)=a_6(q^2,p\cdot q) \epsilon^{\mu\nu\alpha\beta}p_\alpha q_\beta \, .
\end{equation}

\subsection{Vanishing of $c_A$ Term}\label{app:ca}

The three-point correlation function is defined as
\begin{equation}
  G_3^{\mu\nu}(x,y)=\bra{\Omega}|\mathcal{T}\{J_{A}^\mu(x)J_{A}^\nu(y)\mathcal{O}_\pi^{\dagger}(0)\}\ket{\Omega} \, .
  \label{3-pt-correlation-function}
\end{equation}
%
where $J_{A}^\mu(x)$ is given in eq.~\eqref{eq:order-a_current}, and $\mathcal{O}_\pi^{\dagger}(0)=\overline{\psi}(0)\gamma_5\psi(0)=Z_\pi\overline{\psi}^{(0)}(0)\gamma_5\psi^{(0)}(0)$. Neglecting terms proportional to $c_A'$ in Eq.~(\ref{eq:order-a_current}), which will be considered in the next subsection,
\footnote{At $O(a)$, there are no cross-terms between the $c_A$ and $c_A'$ corrections, since these would be proportional to $a^2 c_A c_A'$, so these two effects can be studied separately.} 
one can expand the $O(a)$ improvements to the currents in Eq.~(\ref{3-pt-correlation-function}) as \cite{Bhattacharya_2006}
%
\begin{equation}
\begin{split}
G_3^{\mu\nu}(x,y)&=Z^2(a)Z_\pi\bra{\Omega}|T\bigg\{\bigg(\overline{\Psi}^{(0)}(x)\gamma^\mu\gamma^5 \psi^{(0)}(x)+\overline{\psi}^{(0)}(x)\gamma^\mu\gamma^5 \Psi^{(0)}(x)
\\
&+ac_A \partial^\mu \bigg\{\overline{\Psi}^{(0)}(x)\gamma^5 \psi^{(0)}(x)\bigg\}+ac_A \partial^\mu \bigg\{\overline{\psi}^{(0)}(x)\gamma^5 \Psi^{(0)}(x)\bigg\}\bigg)
\\
&\times\bigg(\overline{\Psi}^{(0)}(y)\gamma^\nu\gamma^5 \psi^{(0)}(y)+\overline{\psi}^{(0)}(y)\gamma^\nu\gamma^5 \Psi^{(0)}(y)
\\
&+ac_A \partial^\nu \bigg\{\overline{\Psi}^{(0)}(y)\gamma^5 \psi^{(0)}(y)\bigg\}+ac_A \partial^\nu \bigg\{\overline{\psi}^{(0)}(y)\gamma^5 \Psi^{(0)}(y)\bigg\}\bigg)
\\
&\times [\overline{\psi}^{(0)}(0)\gamma^5 \psi^{(0)}(0)]^{\dagger}\bigg\}\ket{\Omega}+\mathcal{O}(a^2) \, ,
\end{split}
\end{equation}
%
where $Z(a)=Z_A(1+\tilde{b}_Aa \tilde{m}_{ij})$, and $\tilde{m}_{ij}=(\tilde{m}_i+\tilde{m}_j)/2$. At order $a$, there are two terms proportional to $c_A$, one with the $c_A$ contribution originating from the $J^\mu$ current and the other with $c_A$ from the $J^\nu$ current.  To illustrate that terms proportional to $c_{A}$ vanish, it suffices to investigate one of these two terms.  For this purpose, contribution with $c_{A}$ coming from the improvement of $J^{\nu}$ is chosen:
%
\begin{equation}
G_{3,2}^{\mu\nu}(x,y)\equiv 
Z^2(a)Z_\pi ac_A \bra{\Omega}|T\bigg\{\bigg(\overline{\Psi}^{(0)}(x)\gamma^\mu\gamma^5 \psi^{(0)}(x)\bigg)\bigg(\partial^\nu \bigg\{\overline{\psi}^{(0)}(y)\gamma^5 \Psi^{(0)}(y)\bigg\}\bigg)
[\overline{\psi}^{(0)}(0)\gamma^5 \psi^{(0)}(0)]^{\dagger}\bigg\}\ket{\Omega}+\mathcal{O}(a^2) \, .
\end{equation}
%
The Fourier transform of $G_{3,2}^{\mu\nu}(x,y)$ is denoted $\tilde{G}_{3,2}^{\mu\nu}(p_1,p_2)$. Integrating by parts yields
%
\begin{equation}
\begin{split}
  \tilde{G}_{3,2}^{\mu\nu}(p_1,p_2)=Z^2(a)Z_\pi ac_A ip_2^\nu\int d^4x \, e^{-i p_1\cdot x } \, d^4y e^{-i p_2\cdot y} \bra{\Omega}|T\bigg\{\bigg(\overline{\Psi}^{(0)}(x)\gamma^\mu\gamma^5 \psi^{(0)}(x)\bigg)\bigg(\overline{\psi}^{(0)}(y)\gamma^5 \Psi^{(0)}(y)\bigg)
\\
\times
[\overline{\psi}^{(0)}(0)\gamma^5 \psi^{(0)}(0)]^{\dagger}\bigg\}\ket{\Omega} \, .
\end{split}
\label{matrix-element}
\end{equation}

Consider the most general form of the matrix element in Eq.~(\ref{matrix-element}). Since there is already one factor of $p_2^\nu$, the integral must transform as a vector under Lorentz boosts. Thus, the most general form of $C_{3,2}^{\mu\nu}(p_1,p_2)$ must be
%
\begin{equation}
  \tilde{G}_{3,2}^{\mu\nu}(p_1,p_2)=b_1(p_1^2,p_2^2,p_1\cdot p_2) p_1^\mu p_2^\nu +b_2(p_1^2,p_2^2,p_1\cdot p_2) p_2^\mu p_2^\nu \, .
\end{equation}
%
Using the parity constraints derived previously allows one to conclude that $C_{3,2}^{\mu\nu}(p_1,p_2)$ contains no terms which satisfy these symmetry properties, and therefore it must vanish. The other term proportional to $c_A$ (arising from the correction to $J^\mu$) vanishes analogously.  Thus, $c_A$ terms do not contribute to the $O(a)$ correction.

\subsection{Vanishing of $c_A'$ terms}\label{app:ca-prime}

Neglecting the $c_A$ and $Z_A$ corrections discussed above, the discretized version of the three-point correlator given in Eq.~\eqref{3pt-corr} is given by
\begin{equation}
  \begin{split}
    C_3^{\mu\nu} = \sum_{\mathbf{x}_e, \mathbf{x}_m} \langle &\left[ \overline \psi_u (x_m) \gamma^\nu \gamma^5 \Psi(x_m) - \frac{a}{4} c'_A \left( \overline \psi_u (x_m) \gamma^\nu \gamma^5 (\overrightarrow{D}_\Psi \Psi)(x_m) - (\overline \psi_u \overleftarrow{D}_\psi)(x_m) \gamma^\nu \gamma^5 \Psi(x_m) \right) \right] \\
    &\left[ \overline \Psi(x_e) \gamma^\mu \gamma^5 \psi_d(x_e) - \frac{a}{4}c'_A \left( \overline \Psi(x_e) \gamma^\mu \gamma^5 (\overrightarrow{D}_\psi \psi_d)(x_e) - (\overline \Psi \overleftarrow{D}_\Psi)(x_e) \gamma^\mu \gamma^5 \psi_d(x_e) \right) \right] \\
    &\left[ \overline \psi_d(0) \gamma^5 \psi_u(0) \right] \rangle e^{i\mathbf{p}_e \cdot \mathbf{x}_e} e^{i\mathbf{p}_m \cdot \mathbf{x}_m}
  \end{split}
  \label{contact-terms}
\end{equation}
where the $u$ and $d$ quarks are degenerate and are solely distinguished in order to avoid disconnected diagrams.

Expanding this out gives 
\begin{equation}
  \begin{split}
    C_3^{\mu\nu} &= \sum_{\mathbf{x}_e, \mathbf{x}_m} \left\langle \left[ \overline \psi_u (x_m) \gamma^\nu \gamma^5 \Psi(x_m) \right]\left[ \Psi(x_e) \gamma^\mu \gamma^5 \psi_d (x_e) \right]\left[ \overline \psi_d (0) \gamma^5 \psi_u(0) \right] \right\rangle e^{i\mathbf{p}_e \cdot \mathbf{x}_e} e^{i\mathbf{p}_m \cdot \mathbf{x}_m} \\
    &- a \sum_{\mathbf{x}_e, \mathbf{x}_m} \frac{c_A'}{4} \left\langle \left[ \overline \psi_u (x_m) \gamma^\nu \gamma^5 (\overrightarrow D_\Psi \Psi)(x_m) - (\overline \psi_u \overleftarrow D_\psi)(x_m) \gamma^\nu \gamma^5 \Psi (x_m) \right] \right. \\
    &\hspace{63pt} \left.\left[ \overline \Psi(x_e) \gamma^\mu \gamma^5 \psi_d(x_e) \right]\left[ \overline \psi_d (0) \gamma^5 \psi_u (0) \right] \right\rangle e^{i\mathbf{p}_e \cdot \mathbf{x}_e} e^{i\mathbf{p}_m \cdot \mathbf{x}_m} \\
    &- a \sum_{\mathbf{x}_e, \mathbf{x}_m} \frac{c_A'}{4} \left\langle \left[ \overline \psi_u (x_m) \gamma^\nu \gamma^5 \Psi(x_m) \right] \left[ \overline \Psi(x_e) \gamma^\mu \gamma^5 (\overrightarrow D_\psi \psi_d)(x_e) - (\overline \Psi \overleftarrow D_\Psi)(x_e) \gamma^\mu \gamma^5 \psi_d (x_e) \right] \right. \\
    &\hspace{63pt} \left.\left[ \overline \psi_d (0) \gamma^5 \psi_u (0) \right] \right\rangle e^{i\mathbf{p}_e \cdot \mathbf{x}_e} e^{i\mathbf{p}_m \cdot \mathbf{x}_m} \\
    &+ O(a^2) \, .
  \end{split}
  \label{expanded-contact-terms}
\end{equation}

The first line of Eq.~(\ref{expanded-contact-terms}) is the tree-level contribution studied above.  The second and third lines contain four very similar terms, the first of which is
\begin{equation}
  -a \sum_{\mathbf{x}_e, \mathbf{x}_m} \frac{c_A'}{4} \left\langle \left[ \overline \psi_u (x_m) \gamma^\nu \gamma^5 (\overrightarrow D_\Psi \Psi)(x_m) \right] \left[ \overline \Psi(x_e) \gamma^\mu \gamma^5 \psi_d(x_e) \right]\left[ \overline \psi_d (0) \gamma^5 \psi_u (0) \right] \right\rangle e^{i\mathbf{p}_e \cdot \mathbf{x}_e} e^{i\mathbf{p}_m \cdot \mathbf{x}_m} \, .
\end{equation}
Explicitly writing out all spin, colour, and spacetime indices, this becomes
\begin{equation}
  \begin{split}
- \frac{a c_A'}{4} \sum_{\mathbf{x}_e, \mathbf{x}_m, x} &\left\langle \left[ \overline \psi_u (x_m)_a^\alpha (\gamma^\nu \gamma^5)^{\alpha\beta} D_\Psi (x_m | x)_{ab}^{\beta\gamma} \Psi(x)_b^\gamma \right] \right. \\
&\hspace{6pt}\left. \left[ \overline \Psi(x_e)_c^\delta (\gamma^\mu \gamma^5)^{\delta \varepsilon} \psi_d (x_e)_c^\varepsilon \right] \left[ \overline \psi_d(0)_d^\zeta (\gamma^5)^{\zeta\eta} \psi_u(0)_d^\eta \right]  \right\rangle e^{i\mathbf{p}_e \cdot \mathbf{x}_e} e^{i\mathbf{p}_m \cdot \mathbf{x}_m} \, .
  \end{split}
  \label{explicit-indices}
\end{equation}
Performing the contractions with Wick's theorem gives
\begin{equation}
  \begin{split}
    \frac{ac_A'}{4} \sum_{\mathbf{x}_e, \mathbf{x}_m, x} &\left[ D_u^{-1}(0|x_m)_{da}^{\eta\alpha} \right] \left[ D_d^{-1}(x_e|0)_{cd}^{\varepsilon\zeta} \right] \left[ D_\Psi^{-1}(x|x_e)_{bc}^{\gamma\delta} \right] \left[ D_\Psi (x_m|x)_{ab}^{\beta\gamma} \right] \\
    &\left( \gamma^\nu \gamma^5 \right)^{\alpha\beta} \left( \gamma^\mu \gamma^5 \right)^{\delta\varepsilon} \left( \gamma^5 \right)^{\zeta\eta} e^{i\mathbf{p}_e \cdot \mathbf{x}_e} e^{i\mathbf{p}_m \cdot \mathbf{x}_m} \, .
  \end{split}
  \label{wick-contractions}
\end{equation}
Note that
\begin{equation}
  \sum_x D_\Psi(x_m|x)_{ab}^{\beta\gamma} D_\Psi^{-1}(x|x_e)_{bc}^{\gamma\delta} = \delta^{(4)}(x_m - x_e) \delta^{\beta\delta} \delta_{ac}
  \label{dirac-inverse}
\end{equation}
and thus these terms cannot contribute to this analysis, where contributions from $\tau \equiv \tau_m - \tau_e = 0$ have been explicitly removed.  However, for completeness, it should be noted that one can show that these terms are in fact zero.  With this result, equation (\ref{wick-contractions}) becomes
\begin{align}
  \frac{ac_A'}{4} &\sum_{\mathbf{x}_e, \mathbf{x}_m} \sum_{\mathbf{x}_e, \mathbf{x}_m} e^{i(\mathbf{p}_e + \mathbf{p}_m)\cdot \mathbf{x}_e}\left[ D_u^{-1}(0|x_m)_{da}^{\eta\alpha} \right] \left[ D_d^{-1}(x_e|0)_{cd}^{\varepsilon\zeta} \right] \left[ \delta^{(4)}(x_m-x_e) \delta^{\beta\gamma} \delta_{ac} \right] \left( \gamma^\nu \gamma^5 \right)^{\alpha\beta} \left( \gamma^\mu \gamma^5 \right)^{\delta\varepsilon} \left( \gamma^5 \right)^{\zeta\eta} \\
  &= \frac{ac_A'}{4} \delta(\tau_e - \tau_m) \sum_{\mathbf{x}_e} e^{i(\mathbf{p}_e + \mathbf{p}_m)\cdot \mathbf{x}_e} D^{-1}(0|x_e)_{da}^{\eta\alpha} D^{-1}(x_e|0)_{ad}^{\varepsilon\zeta} \left( \gamma^\nu \gamma^5 \right)^{\alpha\beta} \left( \gamma^\mu \gamma^5 \right)^{\beta\varepsilon} \left( \gamma^5 \right)^{\zeta\eta} \\
  &= \frac{ac_A'}{4} \delta(\tau_e - \tau_m) \sum_{\mathbf{x}_e} e^{i\mathbf{p}_\pi \cdot \mathbf{x}_e} \text{Tr}\left[ D^{-1}(0|x_e) \gamma^\nu \gamma^\mu D^{-1}(x_e|0) \gamma^5 \right] \, .
  \label{pion-b1-correlator}
\end{align}

Under charge conjugation, $\psi \rightarrow C^{-1} \overline \psi^T$ and $\overline \psi \rightarrow -\psi^T C$ (with $C = i \gamma^2 \gamma^4$), so
\begin{equation}
  D^{-1}(x|y) = \langle \psi(x) \overline \psi(y) \rangle \rightarrow C D^{-1}(y|x)^T C^{-1}
  \label{charge-conjugation}
\end{equation}
Further noting that $C\gamma^\mu C^{-1} = -(\gamma^\mu)^T$ and $C\gamma^5 C^{-1} = \left( \gamma^5 \right)^T$, charge conjugation sends the trace in Eq.~(\ref{pion-b1-correlator}) to
\begin{align}
  \text{Tr}\left[ C D^{-1}(x_e|0)^T C^{-1}\gamma^\nu \gamma^\mu C D^{-1}(0|x_e)^T C^{-1} \gamma^5 \right]
  &= \text{Tr}\left[ D^{-1}(x_e|0)^T (\gamma^\nu)^T (\gamma^\mu)^T D^{-1}(0|x_e)^T (\gamma^5)^T \right] \\
  &= \text{Tr}\left[ D^{-1}(0|x_e) \gamma^\mu \gamma^\nu D^{-1}(x_e|0) \gamma^5 \right] \\
  &= -\text{Tr}\left[ D^{-1}(0|x_e) \gamma^\nu \gamma^\mu D^{-1}(x_e|0) \gamma^5 \right]  \, .
  \label{flipped-sign}
\end{align}
Since QCD is invariant under charge conjugation, amplitudes must be similiarly invariant, so this trace must vanish.  The remaining $c_A'$ terms vanish similarly, so there is no need to include the corresponding operators in the definition of the axial currents $J_A^\mu$.



==> definition.tex <==
Before proceeding to describe the numerical lattice determination for
the second Mellin and Gegenbauer moments of $\phi_{\pi} (\xi, \mu)$, a review of the definition of these moments is in order.   The discussion presented here also serves the purpose of setting the conventions and notation that will be used in subsequent calculations.


Conformal symmetry in QCD~\cite{Braun:2003rp} implies that the pion
LCDA can be conveniently studied using the Gegenbauer OPE.  $C$-parity imposes the constraint $\phi_{\pi}
(\xi,\mu) = \phi_{\pi} (-\xi, \mu)$ in the isospin limit, leading to
%
\beq
\label{eq:Gegen_OPE_phi_pi}
\phi_{\pi}(\xi, \mu) = \frac{3}{4} (1 - \xi^{2})
\sum_{n=0,{\mathrm{even}}}^{\infty} \phi_{n}(\mu)
{\mathcal{C}}_{n}^{3/2} (\xi) \, ,
\eeq
%
where ${\mathcal{C}}_{n}^{3/2} (\xi)$ are the Gegenbauer polynomials.  The
Gegenbauer moments, $\phi_{n}(\mu)$, are defined as
%
\beq
\label{eq:Gegen_moment_def}
 \phi_{n}(\mu) = \frac{2 (2n+3)}{3 (n+1)(n+2)} \int_{-1}^{1} d \xi
 \mbox{ } {\mathcal{C}}_{n}^{3/2} (\xi) \phi_{\pi}(\xi, \mu) \, .
\eeq
%
Because of conformal symmetry, the $\phi_{n}(\mu)$ do not mix under the
renormalization group (RG) evolution at one loop.  To this order,
their renormalization scale dependence is~\cite{Efremov:1978rn}
%
\beq
\label{eq:Gegen_moment_one_loop_running}
 \phi_{n} (\mu_{2}) = \phi_{n} (\mu_{1}) \left ( \frac{\alpha_{s}(\mu_{2})}{\alpha_{s}(\mu_{1})} \right
 )^{\gamma_{n}/\beta_{0}} \, ,
\eeq
%
where $\alpha_{s}$ is the strong coupling, $\beta_{0} = 11 - 2N_{f}/3$ ($N_{f}$ being the number of
flavours) is the coefficient of the leading-order (LO) QCD
$\beta$-function, and $\gamma_{n}$ is the anomalous dimension,
%
\beq
\label{eq:Gegen_moment_anomalous_dim}
 \gamma_{n} = \frac{4}{3} \left [ 1 - \frac{2}{(n+1)(n+2)} +4
 \sum_{j=2}^{n+1}j^{-1} \right ] \, .
\eeq
%
Since $\gamma_{n}$ increases monotonically with $n$, one expects that
a truncated version of the OPE in Eq.~(\ref{eq:Gegen_OPE_phi_pi})
can be a good approximation to $\phi_{\pi}(\xi,\mu)$ at large enough
renormalization scales.
In the regime where $\mu \gg \Lambda_{{\mathrm{QCD}}}$ (with
$\Lambda_{{\mathrm{QCD}}}$ being the QCD dynamical scale),  the pion LCDA is dominated by the
zeroth Gegenbauer moment.  
Equations~(\ref{eq:Gegen_moment_one_loop_running}) and (\ref{eq:Gegen_moment_anomalous_dim})  lead to the asymptotic form the pion LCDA,
%
\beq
\label{eq:Phi_pi_asymptotic}
 \lim_{\mu\rightarrow\infty}\phi_{\pi} (\xi, \mu) = \frac{3}{4}
 \left ( 1 - \xi^{2} \right ) \, ,
\eeq
%
where the normalization $\phi_{0} = 1$ has been imposed.



The Gegenbauer moments in Eqs.~(\ref{eq:Gegen_OPE_phi_pi}) and (\ref{eq:Gegen_moment_def}) can be expressed as linear
combinations of the Mellin moments $\la \xi^{n} \ra$, which are defined as
%
\beq
\label{eq:Mellin_moments_def}
 \la \xi^{n} \ra (\mu) = \int_{-1}^{1} d\xi \mbox{ }\xi^{n}
 \phi_{\pi}(\xi,\mu) \, .
\eeq
%
For instance, from Eqs.~(\ref{eq:Gegen_OPE_phi_pi}) and (\ref{eq:Mellin_moments_def}) it is straightforward to obtain
%
\begin{equation}
\label{eq:G_to_M_moments}
 \phi_{0}  = \la \xi^{0} \ra = 1\, , \,\,  \phi_{2} = \frac{7}{12}
 \left ( 5 \la \xi^{2} \ra - \la \xi^{0} \ra \right ) \, , \,\,
 \phi_{4} = \frac{11}{24} \left ( 21 \la \xi^{4}\ra - 14 \la
 \xi^{2}\ra + \la \xi^{0}\ra\right ) \, , \ldots \,  .
\end{equation}
%
In general, knowledge of $\la \xi^{0} \ra$, $\la \xi^{2}\ra$, ...,
$\la \xi^{n} \ra$ is equivalent to that of $\phi_{0}$, $\phi_{2}$, ...,
$\phi_{n}$.  These Mellin moments, $\la \xi^{n} \ra$, can be related to matrix elements of local,
twist-two, operators, 
%
\beq
\label{eq:Mellin_moments_to_ME}
 \la 0 |  \big [ \overline{d}
  \gamma^{\{\mu_0}\gamma_5(i\overset{\leftrightarrow}{D}\vphantom{D}^{\,\mu_1})\dots(i\overset{\leftrightarrow}{D}\vphantom{D}^{\,\mu_n\}})
  u  - {\mathrm{traces}} \big  ] | \pi^{+} (\mathbf{p})
\ra
 =f_{\pi} \expval{\xi^{n}}(\mu^2) \left [ p^{\mu_0}p^{\mu_1}\dots p^{\mu_n}-
 {\mathrm{traces}} \right ] \, ,
\eeq
%
where the Lorentz indices are totally symmetrized, with 
%
\beq
\label{eq:two_way_derivative_def}
\overset{\leftrightarrow}{D}\vphantom{D}^{\,\mu}=\frac{1}{2}(\overset{\rightarrow}{D}\vphantom{D}^{\,\mu}-\overset{\leftarrow}{D}\vphantom{D}^{\,\mu})
\, ,
\eeq
%
and the traces are taken in all possible pairs amongst the Lorentz
indices, $\mu_{0}, \mu_{1}, \ldots, \mu_{n}$.  As discussed in the
last paragraph, from the leading-order result of QCD perturbation
theory, it is natural to expect that knowledge of the first few Gegenbauer
moments allows one to construct $\phi_{\pi} (\xi, \mu)$ reliably at
sufficiently large $\mu$.  This also implies
that obtaining important information about the LCDA at $\mu \gg \Lambda_{{\mathrm{QCD}}}$ is possible from the first few Mellin
moments\footnote{The qualitative feature of low-moment dominance in
  $\phi_{\pi}$ was also argued using QCD sum rules~\cite{Chernyak:1981zz}.}.
This point
can be illustrated by investigating an extreme scenario where one
truncates the Gegenbauer OPE in Eq.~(\ref{eq:Gegen_OPE_phi_pi}) at
$n=2$.  The pion LCDA constructed with this truncated OPE is denoted $\phi_{\pi}^{(2)}(\xi, \mu) $.  Using
Eq.~(\ref{eq:G_to_M_moments}), one obtains
%
\bea
\label{eq:phi_pi_OPE_to_xi2}
\phi_{\pi}^{(2)}(\xi, \mu) &=& \frac{3}{4} (1 - \xi^{2}) \left [
\phi_{0}(\mu) {\mathcal{C}}^{3/2}_{0} (\xi) +\phi_{2}(\mu)
{\mathcal{C}}^{3/2}_{2} (\xi) \right ]\nonumber\\
 &=& \frac{15}{32} \left [ 3 - 7 \la \xi^{2}
\ra (\mu) \right ] + \frac{16}{15} \left [ -5 + 21 \la \xi^{2} \ra (\mu)\right ]
\xi^{2} + \frac{105}{32} \left [ 1 - 5 \la \xi^{2} \ra (\mu)\right ] \xi^{4}
\, .
\eea
%
Figure~\ref{fig:Xi2_pheno} shows the result with $\phi_{\pi}^{(2)}(\xi,
\mu)$ at $\la \xi^{2} \ra (\mu) = 0.2$, 0.25 and 0.3.  
%
\begin{figure}
\centering
\includegraphics[scale=0.6]{graphics/other_plots/xi2_pheno_no_logo.pdf}
\caption{Dependence of $\phi_{\pi}^{(2)}(\xi,
\mu)$, defined in Eq.~(\ref{eq:phi_pi_OPE_to_xi2}), on the values of
$\la \xi^{2} \ra$.  The range of $\la \xi^{2} \ra$ values shown in the
plot covers typical results for this second Mellin moment at $\mu
\sim 2$ GeV from modern lattice
computations.  They lead to consistency with a single-humped or double-humped structure of the DA, and more precise measurements would resolve this.
}
\label{fig:Xi2_pheno}
\end{figure}
%
Note that these
are typical values for this second Mellin moment at $\mu
\sim 2$ GeV from modern lattice
computations~\cite{Del_Debbio_2003, Arthur_2011, 
  Bali:2017gfr, Zhang:2017bzy, Bali:2019dqc}.   This figure demonstrates
that the shape of the pion LCDA can depend strongly upon $\la
\xi^{2}\ra (\mu)$.  Naturally, the inclusion of higher moments will likely reduce the sensitivity to the second moment, but nevertheless, this exercise shows that the second Mellin moment is a phenomenologically interesting quantity.



